Parameter identification in uncertain scalar conservation laws discretized with the discontinuous stochastic Galerkin Scheme

We study an identification problem which estimates the parameters of the underlying random distribution for uncertain scalar conservation laws. The hyperbolic equations are discretized with the so-called discontinuous stochastic Galerkin method, i.e., using a spatial discontinuous Galerkin scheme and a Multielement stochastic Galerkin ansatz in the random space. We assume an uncertain flux or uncertain initial conditions and that a data set of an observed solution is given. The uncertainty is assumed to be uniformly distributed on an unknown interval and we focus on identifying the correct endpoints of this interval. The first-order optimality conditions from the discontinuous stochastic Galerkin discretization are computed on the time-continuous level. Then, we solve the resulting semi-discrete forward and backward schemes with the Runge Kutta method. To illustrate the feasibility of the approach, we apply the method to a stochastic advection and a stochastic equation of Burgers' type. The results show that the method is able to identify the distribution parameters of the random variable in the uncertain differential equation even if discontinuities are present.

==> Images/archiv_sinus.tex <==

\begin{figure}[htb]
	\centering
 \begin{tikzpicture}
  \begin{axis}[width=2\figurewidth, height=\figureheight, xlabel=$\#$Iteration, ylabel=$\xi$, ylabel style = {rotate=-90}, legend style={at={(0.97,0.7)}}] 
   \addplot[mark=none, solid, tuklred, line width=.7pt] file {Images/sinus/sin_xiL.txt};
   \addplot[mark=none, dashed, tuklblue, line width=.8pt] file {Images/sinus/RefxiL.txt};
   \addplot[mark=none, solid, tuklred, line width=.7pt] file {Images/sinus/sin_xiR.txt};
   \addplot[mark=none, dashed, tuklblue, line width=.8pt] file {Images/sinus/RefxiR.txt};
   \legend{$\uncertaintyInt$, $\uncertaintyInt_{\text{Ref}}$}
  \end{axis}
 \end{tikzpicture}
 \caption{Performance of $\xi$ during the optimization process. Example \eqref{eq:initial_sinus}.}
 \label{fig:sinus_xi}
\end{figure}

\begin{figure}[htb]
	\centering
	\begin{subfigure}[b]{0.45\textwidth}
	\begin{tikzpicture}
	\begin{axis}[width=1.3\figurewidth, height=\figureheight, xlabel=$\#$Iteration, ylabel=$\costfun$, ylabel style = {rotate=-90}] 
	\addplot[mark=none, solid, tuklblue, line width=.7pt] file {Images/sinus/sin_J.txt};
	\end{axis}
	\end{tikzpicture}
%	 \subcaption{$\costfun(\solvec,\uncertaintyInt)$}
	\end{subfigure}
%\hspace*{1cm}
%	\begin{subfigure}[b]{0.28\textwidth}
%	\begin{tikzpicture}
%	\begin{axis}[width=\figurewidth, height=\figureheight, xlabel=Iteration, ylabel style = {rotate=-90}] 
%	\addplot[mark=none, solid, tuklblue, line width=.7pt] file {Images/sinus/sin-3_Ju.txt};
%	\end{axis}
%	\end{tikzpicture}
%	\subcaption{$\costfun_\solution$}
%\end{subfigure}
\hspace*{1cm}
	\begin{subfigure}[b]{0.45\textwidth}
	\begin{tikzpicture}
	\begin{axis}[width=1.3\figurewidth, height=\figureheight, xlabel=$\#$Iteration, ylabel=$\costfun_\uncertainty$, ylabel style = {rotate=-90}] 
	\addplot[mark=none, solid, tuklblue, line width=.7pt] file {Images/sinus/sin_Jxi.txt};
	\end{axis}
	\end{tikzpicture}
%	\subcaption{$\costfun_\uncertainty(\uncertaintyInt,\uncertaintyInt_p)$}
\end{subfigure}
	\caption{Cost functional during the optimization process. Example \eqref{eq:initial_sinus}.}
	\label{fig:sinus_J}
\end{figure}

\begin{figure}[htb]
	\centering
	\hspace*{-1cm}
	\begin{minipage}[b]{0.45\textwidth}
		\begin{tikzpicture}
		\begin{axis}[width=1.3\figurewidth, height=\figureheight, xlabel=$\#$Iteration, ylabel=$\|\solution-\solution_D\|_{L_1}$,  y tick label style={ /pgf/number format/.cd, fixed,precision = 6,/tikz/.cd}] 
		\addplot[mark=none, solid, tuklblue, line width=.7pt] file {Images/sinus/sin_u-uD.txt};
		\end{axis}
		\end{tikzpicture}
		\caption{$L_1$ norm of $\solution(\tend) - \solution_D(\tend)$ during the optimization process. Example \eqref{eq:initial_sinus}.}
		\label{fig:sinus_u-uD}
	\end{minipage}
\hspace*{1cm}
\begin{minipage}[b]{0.45\textwidth}
	\begin{tikzpicture}
	\begin{axis}[width=1.3\figurewidth, height=\figureheight, xlabel=$\#$Iteration, ylabel=$\#$Armijo, 	ytick={2,3,4}] 
	\addplot[mark=none, solid, tuklblue, line width=.7pt] file {Images/sinus/sin_Armijo.txt};
	\end{axis}
	\end{tikzpicture}
	\caption{Number of Armijo steps during the optimization process. Example \eqref{eq:initial_sinus}.}
	\label{fig:sinus_armijo}
\end{minipage}
\end{figure}


==> Sections/opticond_advection.tex <==
\section{First order optimality conditions}\label{sec:FOcond}
In this section, we derive the first order optimality conditions of \eqref{eq:OP}.
At first, we restrict the conservation law \eqref{eq:spde} to the one-dimensional hyperbolic linear advection equation
\begin{subequations}\label{eq:LA}
\begin{align}
\frac{\partial}{\partial\timevar}\solution(\timevar ,\x, \uncertainty)+ \advec(\uncertainty) \frac{\partial}{\partial\x} \solution(\timevar ,\x, \uncertainty)&= 0, \quad \quad \text{for} \ \ \x\in\Domain,\, \timevar\in [0,\,\tend],\,\uncertainty\in\SD,\\
\solution(0,\x,\uncertainty) &= \solution_{(0)}(\x,\uncertainty), \quad \quad \text{for} \ \ \x\in\PD,\, \xi\in\SD.
\end{align}
\end{subequations}
The wave speed $\advec=\advec(\uncertainty)$ is uncertain and depending on the uncertainty $\uncertainty$.
In this example, we assume  a uniform distribution $\uncertainty\sim\mathcal{U}(\SD)$. According to \rmref{rem:paramDistr}, we therefore estimate the space $\randomSpace=[\uncertaintyL,\uncertaintyR]$, i.e. the parameters $\uncertaintyL$ and $\uncertaintyR$, which we write as $\uncertaintyInt = \begin{pmatrix}\uncertaintyL\\\uncertaintyR\end{pmatrix}$ with prior estimates $\uncertaintyInt_p = \begin{pmatrix}\uncertaintyL_p\\\uncertaintyR_p\end{pmatrix}$, and set the penalizing cost functional to
$$\costfunxi(\uncertaintyInt,\uncertaintyInt_p)= \frac{\xidelta}{2}\big\|\uncertaintyInt-\uncertaintyInt_p\big\|^2,$$
where we denote by $\|\cdot\|$ the $L_2$-norm. Furthermore, $\xidelta\ll1$ diminishes the impact of $\uncertaintyInt_p$ on the cost functional since $\uncertaintyInt_p$ is only a rough guess of the  true value.

The Lagrange functional corresponding to \eqref{eq:OP} reads
\begin{equation}\label{eq:lagrangian}
\lagrange(\solvec,\uncertaintyInt,\adj) = \sum_{\xsumIndex=0}^{\xdegree}\sum_{\SGsumIndex=0}^\SGtruncorder\, \costfun(\solvec^{\xsumIndex,\SGsumIndex},\uncertaintyInt) 
+ \sum_{\xsumIndex=0}^{\xdegree}\sum_{\SGsumIndex=0}^\SGtruncorder\, \intT\! 
\bigg(\begin{matrix}
\WF(\solvec^{\xsumIndex,\SGsumIndex},\uncertaintyInt)\\[3pt]
\WF_{(0)}(\solvec^{\xsumIndex,\SGsumIndex})
\end{matrix} \bigg)\cdot 
\bigg(\begin{matrix}
\adj^{\xsumIndex,\SGsumIndex}\\[3pt]
\adj^{\xsumIndex,\SGsumIndex}_{(0)}
\end{matrix}\bigg) \,\mathrm{d}\timevar,
\end{equation}
where $\solvec^{\xsumIndex,\SGsumIndex}=\solvec^{\xsumIndex,\SGsumIndex}(\timevar)\in\mathbb{R}^{\ncells\cdot\MEElements}$ contains the vectorized coefficients $\MEDGmoment{\xsumIndex}{\SGsumIndex}{\cellind,\MEIndex}(\timevar)$ for all $\cell{\cellind}\times\randomElement{\MEIndex}$, additionally $\adj^{\xsumIndex,\SGsumIndex}=\adj^{\xsumIndex,\SGsumIndex}(\timevar)\in\mathbb{R}^{\ncells\cdot\MEElements}$ and $\adj^{\xsumIndex,\SGsumIndex}_{(0)}\in\mathbb{R}^{\ncells\cdot\MEElements}$ are the Lagrange multipliers that represent the adjoint state.
%We denote by $\solvec=\solvec(\x,\uncertainty,\timevar)\in\mathbb{R}^{\ncells\cdot\MEElements}$ the vecotirzed values $\localsolution{\cellind}{\cellindR}$.
We denote by $\solvec$ the vectorized values $\solvec^{\xsumIndex,\SGsumIndex}$ and by $\adj$ the vectorized values $\adj^{\xsumIndex,\SGsumIndex}$ and $\adj^{\xsumIndex,\SGsumIndex}_{(0)}$ for all $\xsumIndex=0,\ldots,\xdegree$ and $\SGsumIndex=0,\ldots,\SGtruncorder$.
Moreover, $\WF(\solvec^{\xsumIndex,\SGsumIndex},\uncertaintyInt)\in\mathbb{R}^{\ncells\cdot\MEElements}$ describes the right hand side of the discontinuous stochastic Galerkin formulation given in \eqref{eq:DG}.
For the initial conditions, we obtain the term
$$\WF_{(0)}(\solvec^{\xsumIndex,\SGsumIndex}) = \solvec^{\xsumIndex,\SGsumIndex}(0) - \solvec^{\xsumIndex,\SGsumIndex}_{(0)},$$
which is derived using
\begin{equation}\label{eq:u0}
\big(\solution^{\xsumIndex,\SGsumIndex}_{(0)}\big)_{(\cellind,\MEIndex)} = \frac{1}{\Delta\x\int_{\refcell}\!\int_{\refME}\!\polybasis{\xsumIndex}^2\phi_{\SGsumIndex}^2\,\mathrm{d}\uncertainty\,\mathrm{d}\x}
\,\int_{\cell{\cellind}}\!\int_{\randomElement{\MEIndex}} \solution_{(0)}(\x,\uncertainty)\, \localxiBasisPoly{\SGsumIndex}{\MEIndex}\polybasis{\xsumIndex,\cellind} \, \xiPDFdxi \mathrm{d}\x,
\end{equation}
for $\cellind = 1,\ldots,\ncells$ and $\MEIndex=1,\ldots,\MEElements$. In this example, due to the choice of the uniform distribution for $\uncertainty$, the cost functional reads
$$\costfun(\solvec^{\xsumIndex,\SGsumIndex},\uncertaintyInt) =\frac{1}{2}\big\|\solvec^{\xsumIndex,\SGsumIndex}(\tend) - \udata^{\xsumIndex,\SGsumIndex}\big\|^2 + \frac{\xidelta}{2}\big\|\uncertaintyInt-\uncertaintyInt_p\big\|^2,$$
where the coefficients $\udata^{\xsumIndex,\SGsumIndex}\in\mathbb{R}^{\ncells\cdot\MEElements}$ for each $\xsumIndex=0,\ldots,\xdegree$ and $\SGsumIndex=0,\ldots,\SGtruncorder$ can be calculated from $u_D$  similar to \eqref{eq:u0} as long as the data is available at the same number of spatial cells and \ME{}s -- otherwise we interpolate $u_D$ accordingly. Note that in this case, \eqref{eq:u0} is not depending on the information of the exact interval $D_j$.
%Here, the values $\solution_D\big|_{\cell{\cellind}}$ are interpolated appropriately from $\udata\in\mathbb{R}^d$.
We define $$\costfun(\solvec,\uncertaintyInt):= \sum_{\xsumIndex=0}^{\xdegree}\sum_{\SGsumIndex=0}^\SGtruncorder \costfun(\solvec^{\xsumIndex,\SGsumIndex},\uncertaintyInt).$$

The first-order optimality condition to \eqref{eq:OP} is given by solving 
$$\mathrm{d}\lagrange(\solvec,\uncertaintyInt,\adj) = 0.$$
The derivative w.r.t. the adjoint state $\adj$ results in the state equation, while the derivative w.r.t. the state $\solvec$ yields the adjoint system and the optimality condition is obtained by the derivative w.r.t. the control $\uncertaintyInt$ (c.f. \cite{Hinze2009}).

For these calculations and the linear advection equation \eqref{eq:LA}, we insert the flux function $\flux(\solution) = \advec(\uncertainty)\solution$ into the discontinuous stochastic Galerkin scheme \eqref{eq:DG} using the global Lax-Friedrichs flux \eqref{eq:globalLF}. We obtain
\begin{align*}
\WF(\solvec^{\xsumIndex,\SGsumIndex},\uncertaintyInt)&=
 M_1^{\xsumIndex,\SGsumIndex} \partial_\timevar\solvec^{\xsumIndex,\SGsumIndex} -  
 \sum_{\xsumIndexvar=0}^{\xdegree}\sum_{\SGsumIndexvar=0}^\SGtruncorder M_2^{\xsumIndex,\xsumIndexvar,\SGsumIndex,\SGsumIndexvar} \solvec^{\xsumIndexvar,\SGsumIndexvar} + 
  \sum_{\xsumIndexvar=0}^{\xdegree}\sum_{\SGsumIndexvar=0}^\SGtruncorder M_3^{\xsumIndex,\xsumIndexvar,\SGsumIndex,\SGsumIndexvar} \solvec^{\xsumIndexvar,\SGsumIndexvar},
 \end{align*}
for all $\xsumIndex=0,\ldots,\xdegree$ and $\SGsumIndex=0,\ldots,\SGtruncorder$ and where the matrices $M_1^{\xsumIndex,\SGsumIndex},\, M_2^{\xsumIndex,\xsumIndexvar,\SGsumIndex,\SGsumIndexvar},\, M_3^{\xsumIndex,\xsumIndexvar,\SGsumIndex,\SGsumIndexvar} \in \mathbb{R}^{\ncells\cdot\MEElements\times\ncells\cdot\MEElements}$ are defined by
%\begin{subequations}\label{eq:M}
	\begin{align*}
	M_1^{\xsumIndex,\SGsumIndex} &:= \frac{1}{\Delta\x}\text{diag}\Big(\int_{\cell{\cellind}}\!\polybasis{\xsumIndex,\cellind}\polybasis{\xsumIndex,\cellind}\,\mathrm{d}\x 
	\int_{\randomElement{\MEIndex}}\!\localxiBasisPoly{\SGsumIndex}{\MEIndex}\localxiBasisPoly{\SGsumIndex}{\MEIndex}\,\xiPDFdxi \Big)
	=\text{diag}\Big(\int_{\refcell}\!\polybasis{\xsumIndex}^2\,\mathrm{d}\x 
	\int_{\refME}\!\phi_{\SGsumIndex}^2\,\mathrm{d}\uncertainty \Big)\,,\\
	M_2^{\xsumIndex,\xsumIndexvar,\SGsumIndex,\SGsumIndexvar} &:= 
	\frac{1}{\Delta\x}\text{diag}\Big(\int_{\cell{\cellind}}\!\polybasis{\xsumIndexvar,\cellind}\partial_\x\polybasis{\xsumIndex,\cellind}\,\mathrm{d}\x 
	\int_{\randomElement{\MEIndex}}\!\advec(\uncertainty)\localxiBasisPoly{\SGsumIndexvar}{\MEIndex}\localxiBasisPoly{\SGsumIndex}{\MEIndex}\,\xiPDFdxi \Big)\,,\\
	M_3^{\xsumIndex,\xsumIndexvar,\SGsumIndex,\SGsumIndexvar} & := \frac{1}{2\Delta\x}\text{tridiag}\begin{pmatrix*}[l]
	\hspace*{1.3cm}\polybasis{\xsumIndexvar,\cellind-1}(\x_{\cellind-\frac12}^-)\polybasis{\xsumIndex,\cellind}(\x_{\cellind-\frac12}^+)\int_{\randomElement{\MEIndex}}\!(-\advec(\uncertainty)-\viscosityconstant)\,\localxiBasisPoly{\SGsumIndexvar}{\MEIndex}\localxiBasisPoly{\SGsumIndex}{\MEIndex}\,\xiPDFdxi\\
	\polybasis{\xsumIndexvar,\cellind}(\x_{\cellind+\frac12}^-)\polybasis{\xsumIndex,\cellind}(\x_{\cellind+\frac12}^-)\int_{\randomElement{\MEIndex}}\!(\advec(\uncertainty)+\viscosityconstant)\,\localxiBasisPoly{\SGsumIndexvar}{\MEIndex}\localxiBasisPoly{\SGsumIndex}{\MEIndex}\,\xiPDFdxi\\
	\hspace*{3cm}-\polybasis{\xsumIndexvar,\cellind}(\x_{\cellind-\frac12}^+)\polybasis{\xsumIndex,\cellind}(\x_{\cellind-\frac12}^+)\int_{\randomElement{\MEIndex}}\!(\advec(\uncertainty)-\viscosityconstant)\,\localxiBasisPoly{\SGsumIndexvar}{\MEIndex}\localxiBasisPoly{\SGsumIndex}{\MEIndex}\,\xiPDFdxi\\
	\hspace*{1.5cm}\polybasis{\xsumIndexvar,\cellind+1}(\x_{\cellind+\frac12}^+)\polybasis{\xsumIndex,\cellind}(\x_{\cellind+\frac12}^-)\int_{\randomElement{\MEIndex}}\!(\advec(\uncertainty)-\viscosityconstant)\,\localxiBasisPoly{\SGsumIndexvar}{\MEIndex}\localxiBasisPoly{\SGsumIndex}{\MEIndex}\,\xiPDFdxi\\
	\end{pmatrix*}\,.
	\end{align*}
%\end{subequations}
Note that the \ME{}s $\randomElement{\MEIndex}$ and $\xiPDF$ are depending on the parameters $\uncertaintyInt$. The indices in the matrices run from $\cellind=1,\ldots,\ncells$ and $\MEIndex=1,\ldots,\MEElements$.

For any directions $\directionxi\in\mathbb{R}^2$, $\directionhk=\directionhk(\timevar)\in\mathbb{R}^{\ncells\cdot\MEElements}$, where $\direction$ denotes the vectorized values $\directionhk$, we obtain the following Gâteaux derivatives of the cost functional
\begin{align*}
	\mathrm{d}_{\solvec}  \costfun(\solvec,\uncertaintyInt)[\direction]
	& = \sum_{\xsumIndex=0}^{\xdegree}\sum_{\SGsumIndex=0}^\SGtruncorder (\solvec^{\xsumIndex,\SGsumIndex}(\tend)-\solvec^{\xsumIndex,\SGsumIndex}_D)\cdot \directionhk(\tend),\\[4pt]
	 \mathrm{d}_{\uncertaintyInt} \costfun(\solvec,\uncertaintyInt)[\directionxi] 
	& = \xidelta\,(\uncertaintyInt-\uncertaintyInt_p)\cdot\directionxi.
\end{align*}

The directional derivatives for the second part of the Lagrangian \eqref{eq:lagrangian} read
\begin{align*}
	 &\intT\!  \mathrm{d}_{\solvec} \sum_{\xsumIndex=0}^{\xdegree}\sum_{\SGsumIndex=0}^\SGtruncorder \bigg(\begin{matrix}
	\WF(\solvec^{\xsumIndex,\SGsumIndex},\uncertaintyInt)\\[3pt]
	\WF_{(0)}(\solvec^{\xsumIndex,\SGsumIndex})
	\end{matrix}\bigg) [\direction] \cdot \bigg(\begin{matrix}
	\adj^{\xsumIndex,\SGsumIndex}\\[3pt]
	\adj^{\xsumIndex,\SGsumIndex}_{(0)}
	\end{matrix}\bigg) \mathrm{d}\timevar \\[4pt]
	& \hspace*{1.7cm}= \sum_{\xsumIndex=0}^{\xdegree}\sum_{\SGsumIndex=0}^\SGtruncorder \intT\! 
	M_1^{\xsumIndex,\SGsumIndex} \partial_\timevar \directionhk \cdot \adj^{\xsumIndex,\SGsumIndex} 
	+ \sum_{\xsumIndexvar=0}^{\xdegree}\sum_{\SGsumIndexvar=0}^\SGtruncorder \big(M_3^{\xsumIndexvar,\xsumIndex,\SGsumIndexvar,\SGsumIndex} - M_2^{\xsumIndexvar,\xsumIndex,\SGsumIndexvar,\SGsumIndex}\big)\, \directionhkvar \cdot \adj^{\xsumIndexvar,\SGsumIndexvar}  \,\mathrm{d}\timevar +  \directionhk(0)\cdot\adj^{\xsumIndex,\SGsumIndex}_{(0)}, \\[5pt]
	&\intT\! \mathrm{d}_{\uncertaintyInt} \bigg(\begin{matrix}
	\WF(\solvec^{\xsumIndex,\SGsumIndex},\uncertaintyInt)\\[3pt]
	\WF_{(0)}(\solvec^{\xsumIndex,\SGsumIndex})
	\end{matrix}\bigg)[\directionxi] \cdot 
	\bigg(\begin{matrix}
	\adj^{\xsumIndex,\SGsumIndex}\\[3pt]
	\adj^{\xsumIndex,\SGsumIndex}_{(0)}
	\end{matrix}\bigg) \mathrm{d}\timevar \\[4pt]
	& \hspace*{1.7cm} = \intT\! \bigg(\Big(
	\sum_{\xsumIndexvar=0}^{\xdegree}\sum_{\SGsumIndexvar=0}^\SGtruncorder \partial_{\uncertaintyInt} \big(M_3^{\xsumIndex,\xsumIndexvar,\SGsumIndex,\SGsumIndexvar} \solvec^{\xsumIndexvar,\SGsumIndexvar}\big)
	- \partial_{\uncertaintyInt} \big(M_2^{\xsumIndex,\xsumIndexvar,\SGsumIndex,\SGsumIndexvar} \solvec^{\xsumIndexvar,\SGsumIndexvar}\big) \Big) \cdot \directionxi \bigg) \cdot\adj^{\xsumIndex,\SGsumIndex} 
	- \Big(\partial_{\uncertaintyInt}\solvec^{\xsumIndex,\SGsumIndex}_{(0)} \cdot \directionxi\Big) \cdot \adj^{\xsumIndex,\SGsumIndex}_{(0)} \,\mathrm{d}\timevar,
\end{align*}
with Lagrange multipliers $\adj^{\xsumIndex,\SGsumIndex}\in\mathbb{R}^{\ncells\cdot\MEElements}$ for $\xsumIndex=0,\ldots,\xdegree$ and $\SGsumIndex=0,\ldots,\SGtruncorder$.
Using \rmref{rem:refCell} yields
	\begin{align*}
\partial_{\uncertaintyInt}\big(M_1^{\xsumIndex,\SGsumIndex}\solvec^{\xsumIndex,\SGsumIndex}\big) &=\partial_{\uncertaintyInt}\bigg( \text{diag}\Big(\int_{\refcell}\!\polybasis{\xsumIndex}^2\,\mathrm{d}\x 
\int_{\refME}\!\phi_{\SGsumIndex}^2\,\mathrm{d}\uncertainty \Big)\,\solvec^{\xsumIndex,\SGsumIndex}\bigg)=0,\\
\partial_{\uncertaintyR}\big(M_2^{\xsumIndex,\xsumIndexvar,\SGsumIndex,\SGsumIndexvar}\solvec^{\xsumIndexvar,\SGsumIndexvar}\big) &= 
\text{diag}\bigg(\int_{\refcell}\!\polybasis{\xsumIndexvar}\partial_\x\polybasis{\xsumIndex}\,\mathrm{d}\x 
\int_{\refME}\!\advec'\Big(\big(\uncertaintyR-\uncertaintyL\big)\frac{\big(\uncertainty+\MEIndex-\frac12\big)}{\MEElements}+\uncertainty_L\Big)\Big(\frac{\uncertainty+\MEIndex-\frac12}{\MEElements}\Big)
\phi_{\SGsumIndexvar}\phi_{\SGsumIndex}\,\mathrm{d}\uncertainty \bigg)\,\solvec^{\xsumIndexvar,\SGsumIndexvar},
\end{align*}
where $\partial_{\uncertaintyL}\big(M_2^{\xsumIndex,\xsumIndexvar,\SGsumIndex,\SGsumIndexvar}\solvec^{\xsumIndexvar,\SGsumIndexvar}\big)$ and $\partial_{\uncertaintyInt}\big(M_3^{\xsumIndex,\xsumIndexvar,\SGsumIndex,\SGsumIndexvar}\solvec^{\xsumIndexvar,\SGsumIndexvar}\big)$ follow analogously. Furthermore, we have
$$\partial_{\uncertaintyR}\big(\solvec^{\xsumIndex,\SGsumIndex}_{(0)}\big) = \big(M_1^{\xsumIndex,\SGsumIndex}\big)^{-1}
\text{diag}\bigg(\int_{\refcell}\!\int_{\refME}\!\solution_{(0)}'\Big(\x\,\Delta\x+\x_i,\,\big(\uncertaintyR-\uncertaintyL\big)\frac{\big(\uncertainty+\MEIndex-\frac12\big)}{\MEElements}+\uncertainty_L\Big)\Big(\frac{\uncertainty+\MEIndex-\frac12}{\MEElements}\Big)\polybasis{\xsumIndex}\phi_{\SGsumIndex}\,\mathrm{d}\uncertainty\mathrm{d}\x\bigg) .$$
Here, $\solution_{(0)}'$ describes the derivative of $\solution_{(0)}$ w.r.t. the second argument.
\begin{remark}
	In order to derive $\partial_{\uncertaintyInt}\big(M_2^{\xsumIndex,\xsumIndexvar,\SGsumIndex,\SGsumIndexvar}\solvec^{\xsumIndexvar,\SGsumIndexvar}\big)$ and $\partial_{\uncertaintyInt}\big(\solvec^{\xsumIndex,\SGsumIndex}_{(0)}\big)$,  the functions $\advec(\xi)$ and $\solution_{(0)}(\x,\uncertainty)$ have to be differentiable with respect to $\uncertainty$. 
\end{remark}
Using integration by parts we obtain the following result.
\begin{theorem}
Let $\big(\uncertaintyInt_*,(\solvec^{\xsumIndex,\SGsumIndex}_*)_{\xsumIndex=0:\xdegree,\SGsumIndex=0:\SGtruncorder}\big)$ be an optimal pair for \eqref{eq:OP}. Then we have the following first order optimality condition 
\begin{align}\label{eq:opticond}
\intT\! \Big(\sum_{\xsumIndex,\xsumIndexvar=0}^{\xdegree}\sum_{\SGsumIndex,\SGsumIndexvar=0}^\SGtruncorder \partial_{\uncertaintyInt} \big(M_3^{\xsumIndex,\xsumIndexvar,\SGsumIndex,\SGsumIndexvar} \solvec_*^{\xsumIndexvar,\SGsumIndexvar}\big)
&- \partial_{\uncertaintyInt} \big(M_2^{\xsumIndex,\xsumIndexvar,\SGsumIndex,\SGsumIndexvar} \solvec_*^{\xsumIndexvar,\SGsumIndexvar}\big) \Big) \cdot\adj^{\xsumIndex,\SGsumIndex}\,\mathrm{d}\timevar \nonumber\\[2pt]
&+  \partial_{\uncertaintyInt}\solvec^{\xsumIndex,\SGsumIndex}_{(0)} \cdot \big(M_1^{\xsumIndex,\SGsumIndex} \adj^{\xsumIndex,\SGsumIndex}(0)\big)
+  \xidelta\,(\uncertaintyInt_*-\uncertaintyInt_p) = 0,
\end{align}
for all $\uncertaintyInt\in\mathbb{R}^2$ and $\adj^{\xsumIndex,\SGsumIndex} $ satisfies the adjoint problem given by
\begin{equation}\label{eq:adjsys}
	M_1^{\xsumIndex,\SGsumIndex} \,\partial_\timevar \adj^{\xsumIndex,\SGsumIndex}  
	= \sum_{\xsumIndexvar=0}^{\xdegree}\sum_{\SGsumIndexvar=0}^\SGtruncorder \big(M_3^{\xsumIndexvar,\xsumIndex,\SGsumIndexvar,\SGsumIndex} - M_2^{\xsumIndexvar,\xsumIndex,\SGsumIndexvar,\SGsumIndex}\big)^T\,\adj^{\xsumIndexvar,\SGsumIndexvar},
\end{equation}
for $\xsumIndex=0,\ldots,\xdegree$ and $\SGsumIndex=0,\ldots,\SGtruncorder$ with terminal condition $M_1^{\xsumIndex,\SGsumIndex}\adj^{\xsumIndex,\SGsumIndex}(\tend) = (\solvec^{\xsumIndex,\SGsumIndex}_D-\solvec_*^{\xsumIndex,\SGsumIndex})$.
\end{theorem}
\begin{proof} For the optimal pair, we have $\mathrm{d}_\solvec \lagrange(\solvec,\uncertaintyInt,\adj) =0$, where
\begin{align*}
	\intT \!M_1^{\xsumIndex,\SGsumIndex}\partial_t\directionhk\cdot\adj^{\xsumIndex,\SGsumIndex}\,\mathrm{d}\timevar 
	= \intT\! \partial_t\big(M_1^{\xsumIndex,\SGsumIndex}\directionhk\big)\cdot\adj^{\xsumIndex,\SGsumIndex}\,\mathrm{d}\timevar  
	&= \big[\directionhk\cdot\big(M_1^{\xsumIndex,\SGsumIndex}\big)^T\adj^{\xsumIndex,\SGsumIndex}\big]_0^T - \intT\!\directionhk\cdot\big(M_1^{\xsumIndex,\SGsumIndex}\big)^T\partial_\timevar\adj^{\xsumIndex,\SGsumIndex}\,\mathrm{d}\timevar,\\
		\intT \big(M_3^{\xsumIndex,\xsumIndexvar,\SGsumIndex,\SGsumIndexvar} - M_2^{\xsumIndex,\xsumIndexvar,\SGsumIndex,\SGsumIndexvar}\big)\directionhkvar\cdot\adj^{\xsumIndexvar,\SGsumIndexvar} \,\mathrm{d}\timevar
	&= \intT \directionhkvar\cdot\big(M_3^{\xsumIndex,\xsumIndexvar,\SGsumIndex,\SGsumIndexvar} - M_2^{\xsumIndex,\xsumIndexvar,\SGsumIndex,\SGsumIndexvar}\big)^T\adj^{\xsumIndexvar,\SGsumIndexvar} \,\mathrm{d}\timevar.
\end{align*}
Choosing smooth functions with $\directionhk(0)=\directionhk(T)=0$ and $\directionhk(t) \ne 0$ for $t\in (0,T)$ as test functions, and using the symmetry of $M_1^{\xsumIndex,\SGsumIndex}$, we obtain \eqref{eq:adjsys}. Bear in mind the swap of the indices $\xsumIndex$ and $\xsumIndexvar$ such as $\SGsumIndex$ and $\SGsumIndexvar$.
Choosing $\directionhk$ smooth with $\directionhk([0,T))=0 $ yields the terminal condition, where $M_1^{\xsumIndex,\SGsumIndex}$ has full rank thus is invertible. Additionally, using $\directionhk((0,T])=0 $,  we have $\adj^{\xsumIndex,\SGsumIndex}_{(0)} = M_1^{\xsumIndex,\SGsumIndex}\adj^{\xsumIndex,\SGsumIndex}(0)$, together with $\mathrm{d}_{\uncertaintyInt} \lagrange(\solvec,\uncertaintyInt,\adj) =0$ this gives \eqref{eq:opticond}.
\end{proof}
Note that if the advection $\advec(\uncertainty)$ is not depending on $\uncertainty$, the optimality condition \eqref{eq:opticond} only contains the optimization in the uncertain initial condition through the second term $\partial_{\uncertaintyInt}\solvec^{\xsumIndex,\SGsumIndex}_{(0)} \cdot \big(M_1^{\xsumIndex,\SGsumIndex}\adj^{\xsumIndex,\SGsumIndex}(0)\big)$ and the other way around.

\subsection{Reduced Cost Functional}
For the numerical solution of our optimal control problem we need to introduce the reduced cost functional $\redcostfun(\uncertaintyInt)$ and its derivative in order to formulate a steepest descent method. We denote by $$\controltostate(\uncertaintyInt)=\solvec$$ the control-to-state operator describing the solution of the linear advection equation depending on $\uncertaintyInt$, that is deduced through application of the discontinuous stochastic Galerkin scheme \eqref{eq:DG}. The existence and uniqueness of solutions is discussed in \rmref{rem:existunique}. We write \begin{equation}\label{eq:redcostfun}\redcostfun(\uncertaintyInt)=\costfun(\controltostate(\uncertaintyInt),\uncertaintyInt).\end{equation}
We assume that the control-to-state operator is Gâteaux differentiable, otherwise the so called shift derivative has to be introduced, for more information see \cite{Hajian2019,Ulbrich2001}.
%Therefore a different approach in defining a derivative of the control-to-state map, called shift derivative, is derived which leads to Fr´echet differentiability of the objective functional.
Additionally, we define 
$$ \Fvar(\solvec,\uncertaintyInt,\adj) := \sum_{\xsumIndex=0}^{\xdegree}\sum_{\SGsumIndex=0}^\SGtruncorder \bigg(\begin{matrix}
\WF(\solvec^{\xsumIndex,\SGsumIndex},\uncertaintyInt)\\[3pt]
\WF_{(0)}(\solvec^{\xsumIndex,\SGsumIndex})
\end{matrix}\bigg) \cdot \bigg(\begin{matrix}
\adj^{\xsumIndex,\SGsumIndex}\\[3pt]
\adj^{\xsumIndex,\SGsumIndex}_{(0)}
\end{matrix}\bigg).$$
Analogous to \cite{Hinze2009,Totzeck}, using  $\Fvar(\solvec,\uncertaintyInt,\adj)=0$, we obtain 
$$0 = \mathrm{d}_{\uncertaintyInt}\Fvar(\controltostate(\uncertaintyInt),\uncertaintyInt,\adj)
=\mathrm{d}_\solvec\Fvar(\controltostate(\uncertaintyInt),\uncertaintyInt,\adj)[\mathrm{d}\controltostate(\uncertaintyInt)] 
+ \mathrm{d}_{\uncertaintyInt}\Fvar(\controltostate(\uncertaintyInt),\uncertaintyInt,\adj).$$
The derivative of the Lagragian w.r.t. the state $\solvec$ yields
$$\mathrm{d}_\solvec\Fvar(\solvec,\uncertaintyInt,\adj)^*=-\mathrm{d}_\solvec\costfun(\solvec,\uncertaintyInt).$$
With these equations, the  Gâteaux derivative of the reduced cost functional in arbitrary direction $\directionxi\in\mathbb{R}^2$ is given by
\begin{subequations}\label{eq:derredcostfun}
\begin{align}
\mathrm{d}\redcostfun(\uncertaintyInt)[\directionxi]&=\mathrm{d}_\solvec\costfun(\solvec,\uncertaintyInt)\cdot\mathrm{d}\controltostate(\uncertaintyInt)[\directionxi] + \mathrm{d}_{\uncertaintyInt}\costfun(\solvec,\uncertaintyInt)[\directionxi]\\
%&=-\mathrm{d}_\solvec\Fvar(\solvec,\uncertaintyInt)^*[\adj] \cdot\mathrm{d}\controltostate(\uncertaintyInt)[\directionxi] + \mathrm{d}_{\uncertaintyInt}\costfun(\solvec,\uncertaintyInt)[\directionxi]\\
&=\mathrm{d}_{\uncertaintyInt}\Fvar(\controltostate(\uncertaintyInt),\uncertaintyInt,\adj) \cdot \directionxi + \mathrm{d}_{\uncertaintyInt}\costfun(\solvec,\uncertaintyInt)[\directionxi]\\
&=\mathrm{d}_{\uncertaintyInt}\lagrange(\solvec,\uncertaintyInt,\adj) \cdot  \directionxi ,
\end{align}
\end{subequations}
which corresponds to the first order optimality condition from \eqref{eq:opticond}.
